Multimodal sparse representation learning and applications

Unsupervised methods have proven effective for discriminative tasks in a single-modality scenario. In this paper, we present a multimodal framework for learning sparse representations that can capture semantic correlation between modalities. The framework can model relationships at a higher level by forcing the shared sparse representation. In particular, we propose the use of joint dictionary learning technique for sparse coding and formulate the joint representation for concision, cross-modal representations (in case of a missing modality), and union of the cross-modal representations. Given the accelerated growth of multimodal data posted on the Web such as YouTube, Wikipedia, and Twitter, learning good multimodal features is becoming increasingly important. We show that the shared representations enabled by our framework substantially improve the classification performance under both unimodal and multimodal settings. We further show how deep architectures built on the proposed framework are effective for the case of highly nonlinear correlations between modalities. The effectiveness of our approach is demonstrated experimentally in image denoising, multimedia event detection and retrieval on the TRECVID dataset (audio-video), category classification on the Wikipedia dataset (image-text), and sentiment classification on PhotoTweet (image-text).

==> prelim.tex <==
\section{Unimodal Feature Learning}
Approaches of this paper are based from sparse coding, an unsupervised learning method. we build on sparse coding as the basic means to extract features from input data.

\subsection{Sparse Coding}
Given an input $\mathbf{x} \in \mathbb{R}^N$, sparse coding solves for a representation (sparse code) $\mathbf{y} \in \mathbb{R}^K$ in the following optimization problem:
\begin{equation}
\label{eq:bp}
\min_{\mathbf{y}}\Arrowvert \mathbf{x}-\mathbf{D}\mathbf{y} \Arrowvert_{2}^{2} + \lambda \cdot \psi (\mathbf{y})
\end{equation} Here, $\mathbf{x}$ is interpreted as a linear combination of basis vectors in an overcomplete dictionary $\mathbf{D} \in \mathbb{R}^{N \times K}$ ($K \gg N$). The solution $\mathbf{y}$ contains the linear combination coefficients regularized by the sparsity-inducing second term of Eq.~(\ref{eq:bp}) for some $\lambda > 0$. 

Sparse coding employs $\ell_0$- or $\ell_1$-norm of $\mathbf{y}$ as $\psi(.)$. Because $\ell_0$-norm of a vector is the number of its nonzero elements, it precisely fits the regularization purpose of sparse coding. Finding the $\ell_0$-minimum solution for Eq.~(\ref{eq:bp}), however, is known to be NP-hard. The $\ell_1$-minimization known as Basis Pursuit \cite{bp} or LASSO \cite{lasso} is often preferred. Recently, it is known that the $\ell_0$-based greedy algorithms such as Orthogonal Matching Pursuit (OMP) \cite{tropp_2007} can run fast. For this project, our default choice for sparse coding is OMP.

How can we learn a dictionary $\mathbf{D}$ of basis vectors for sparse coding? This is done by an unsupervised, data-driven process incorporating two separate optimizations. It first computes sparse code for each training example (unlabeled) using the current dictionary. Then, the reconstruction error from the computed sparse codes is used to update each basis vector in the dictionary. For this paper, we use K-SVD algorithm \cite{aharon_2006} for dictionary learning.

